ForecastBench: A Dynamic Benchmark of AI Forecasting Capabilities

Forecasts of future events are essential inputs into informed decision-making. Machine learning (ML) systems have the potential to deliver forecasts at scale, but there is no framework for evaluating the accuracy of ML systems on a standardized set of forecasting questions. To address this gap, we introduce ForecastBench: a dynamic benchmark that evaluates the accuracy of ML systems on an automatically generated and regularly updated set of 1,000 forecasting questions. To avoid any possibility of data leakage, ForecastBench is comprised solely of questions about future events that have no known answer at the time of submission. We quantify the capabilities of current ML systems by collecting forecasts from expert (human) forecasters, the general public, and LLMs on a random subset of questions from the benchmark ($N=200$). While LLMs have achieved super-human performance on many benchmarks, they perform less well here: expert forecasters outperform the top-performing LLM ($p$-value $<0.001$). We display system and human scores in a public leaderboard at www.forecastbench.org.

==> figures/forecasting_timeline.tex <==
\begin{figure}[htb]
    \centering
\begin{tikzpicture}[x=1cm, y=1cm, font=\small]
  \definecolor{lightblue}{RGB}{173, 216, 230}
  \definecolor{lightpink}{RGB}{255, 182, 193}

  \node (forecasts) [multidocument,outer sep=1pt] at (13.1,0) {Forecasts};

  \draw[fill=lightblue,draw=lightblue,opacity=0.5] (1, 0) rectangle (12, -0.5);
  \node[align=center] at (6.55, -0.25) {Human forecast period};

  \begin{scope}
    \path[fill=lightpink, pattern=north east lines, pattern color=lightpink] (9, 0) rectangle (12, -0.5);
  \end{scope}
  \node[align=center] at (10.5, -0.25) {LLM forecast period};  

  % Main timeline
  \draw[thick, -{>[scale=1]},-latex'] (0, 0) -- (forecasts.west);

  % D-10
  \draw[thick] (1, -0.5) -- (1, 0.4);
  \node[below, align=center] at (1, -0.5) {LLM \& Human\\question sets\\created};
  \node[above, align=center] at (1, 0.4) {$D-10$\\\texttt{0:00} UTC};

  % D
  \draw[thick] (9, -0.5) -- (9, 0.4);
  \node[below, align=center] at (9, -0.5) {LLM question set\\ released};
  \node[above, align=center] at (9, 0.4) {$D$\\\texttt{0:00} UTC};

  % D
  \draw[thick] (12, -0.5) -- (12, 0.4);
  \node[below, align=center] at (12, -0.5) {LLM \& Human\\forecasts due};
  \node[above, align=center] at (12, 0.4) {\texttt{23:59} UTC};
\end{tikzpicture}
   \caption{Timeline from question set generation to forecast due date, $D$.}
    \label{fig:question_set_timeline}
\end{figure}

==> figures/nightly_question_bank_update.tex <==
\begin{figure}[htb]
    \centering
\begin{tikzpicture}
\node (start) [start] at (-0.3,0) {Daily, \texttt{0:00} UTC};
\node (questions) [process] at (3,0) {Update Questions};
\node (question_files_outer_sep_top) [multidocument,outer sep=4.2pt] at (3,-1.12) {Question Files};
\node (question_files_outer_sep_bottom) [multidocument,outer sep=2.4pt] at (3,-1.12) {Question Files};
\node (resolutions) [process] at (6.5,0) {Update Resolutions};
\node (resolution_files_outer_sep_top) [multidocument,outer sep=4.2pt] at (6.5,-1.1) {Resolution Files};
\node (resolution_files_outer_sep_bottom) [multidocument,outer sep=2.4pt] at (6.5,-1.1) {Resolution Files};
\node (metadata) [process] at (10,0) {Update Metadata};
\node (metadata_file) [singledocument] at (10,-0.95) {Metadata File};
\node (metadata_file_outer_sep) [singledocument,outer sep=2.4pt] at (10,-0.95) {Metadata File};
\node (question_bank) [database] at (6.5,-2.5) {Question\\Bank};
\draw [connector] (start) -- (questions);
\draw [connector] (questions) -- (question_files_outer_sep_top);
\draw [connector] (questions) -- (resolutions);
\draw [connector] (resolutions) -- (resolution_files_outer_sep_top);
\draw [connector] (resolutions) -- (metadata);
\draw [connector] (metadata) -- (metadata_file);
\draw [connector] (metadata_file_outer_sep.south) --  (question_bank.east) ;
\draw [connector] (resolution_files_outer_sep_bottom.south) --  (question_bank.north) ;
\draw [connector] (question_files_outer_sep_bottom.south) --  (question_bank.west) ;
\end{tikzpicture}
   \caption{The automated system that pulls questions from forecasting platforms and datasets for question generation from data providers.}
    \label{fig:question_processing}
\end{figure}

==> figures/sampling_question_sets.tex <==
\begin{figure}[htb]
    \centering
\begin{tikzpicture}
\node (start) [start] at (0,-.5) {Every other Sunday,\\\texttt{0:00} UTC};
\node (sample_questions) [process] at (4,-.5){Sample Questions};
\node (question_bank) [database] at (4,-2) {Question\\Bank};
\node (lm_question_set) [singledocument,align=center,font=\small] at (8,0) { \ \ LLM Question Set \ \ \\(1,000 Questions)};
\node (public_question_set) [singledocument,align=center,font=\small] at (8,-1.25) {Public Question Set\\(200 Questions)};
\draw [connector] (start) -- (sample_questions);
\draw [connector] (question_bank) -- (sample_questions);
\draw [connector] (sample_questions.east) -- (lm_question_set.west);
\draw [connector] (sample_questions.east) -- (public_question_set.west);
\end{tikzpicture}
   \caption{We sample from the question bank every two weeks to produce question sets.}
    \label{fig:creating_question_sets}
\end{figure}

==> math_commands.tex <==
%%%%% NEW MATH DEFINITIONS %%%%%

\usepackage{amsmath,amsfonts,bm}

% Mark sections of captions for referring to divisions of figures
\newcommand{\figleft}{{\em (Left)}}
\newcommand{\figcenter}{{\em (Center)}}
\newcommand{\figright}{{\em (Right)}}
\newcommand{\figtop}{{\em (Top)}}
\newcommand{\figbottom}{{\em (Bottom)}}
\newcommand{\captiona}{{\em (a)}}
\newcommand{\captionb}{{\em (b)}}
\newcommand{\captionc}{{\em (c)}}
\newcommand{\captiond}{{\em (d)}}

% Highlight a newly defined term
\newcommand{\newterm}[1]{{\bf #1}}


% Figure reference, lower-case.
\def\figref#1{figure~\ref{#1}}
% Figure reference, capital. For start of sentence
\def\Figref#1{Figure~\ref{#1}}
\def\twofigref#1#2{figures \ref{#1} and \ref{#2}}
\def\quadfigref#1#2#3#4{figures \ref{#1}, \ref{#2}, \ref{#3} and \ref{#4}}
% Section reference, lower-case.
\def\secref#1{section~\ref{#1}}
% Section reference, capital.
\def\Secref#1{Section~\ref{#1}}
% Reference to two sections.
\def\twosecrefs#1#2{sections \ref{#1} and \ref{#2}}
% Reference to three sections.
\def\secrefs#1#2#3{sections \ref{#1}, \ref{#2} and \ref{#3}}
% Reference to an equation, lower-case.
\def\eqref#1{equation~\ref{#1}}
% Reference to an equation, upper case
\def\Eqref#1{Equation~\ref{#1}}
% A raw reference to an equation---avoid using if possible
\def\plaineqref#1{\ref{#1}}
% Reference to a chapter, lower-case.
\def\chapref#1{chapter~\ref{#1}}
% Reference to an equation, upper case.
\def\Chapref#1{Chapter~\ref{#1}}
% Reference to a range of chapters
\def\rangechapref#1#2{chapters\ref{#1}--\ref{#2}}
% Reference to an algorithm, lower-case.
\def\algref#1{algorithm~\ref{#1}}
% Reference to an algorithm, upper case.
\def\Algref#1{Algorithm~\ref{#1}}
\def\twoalgref#1#2{algorithms \ref{#1} and \ref{#2}}
\def\Twoalgref#1#2{Algorithms \ref{#1} and \ref{#2}}
% Reference to a part, lower case
\def\partref#1{part~\ref{#1}}
% Reference to a part, upper case
\def\Partref#1{Part~\ref{#1}}
\def\twopartref#1#2{parts \ref{#1} and \ref{#2}}

\def\ceil#1{\lceil #1 \rceil}
\def\floor#1{\lfloor #1 \rfloor}
\def\1{\bm{1}}
\newcommand{\train}{\mathcal{D}}
\newcommand{\valid}{\mathcal{D_{\mathrm{valid}}}}
\newcommand{\test}{\mathcal{D_{\mathrm{test}}}}

\def\eps{{\epsilon}}


% Random variables
\def\reta{{\textnormal{$\eta$}}}
\def\ra{{\textnormal{a}}}
\def\rb{{\textnormal{b}}}
\def\rc{{\textnormal{c}}}
\def\rd{{\textnormal{d}}}
\def\re{{\textnormal{e}}}
\def\rf{{\textnormal{f}}}
\def\rg{{\textnormal{g}}}
\def\rh{{\textnormal{h}}}
\def\ri{{\textnormal{i}}}
\def\rj{{\textnormal{j}}}
\def\rk{{\textnormal{k}}}
\def\rl{{\textnormal{l}}}
% rm is already a command, just don't name any random variables m
\def\rn{{\textnormal{n}}}
\def\ro{{\textnormal{o}}}
\def\rp{{\textnormal{p}}}
\def\rq{{\textnormal{q}}}
\def\rr{{\textnormal{r}}}
\def\rs{{\textnormal{s}}}
\def\rt{{\textnormal{t}}}
\def\ru{{\textnormal{u}}}
\def\rv{{\textnormal{v}}}
\def\rw{{\textnormal{w}}}
\def\rx{{\textnormal{x}}}
\def\ry{{\textnormal{y}}}
\def\rz{{\textnormal{z}}}

% Random vectors
\def\rvepsilon{{\mathbf{\epsilon}}}
\def\rvtheta{{\mathbf{\theta}}}
\def\rva{{\mathbf{a}}}
\def\rvb{{\mathbf{b}}}
\def\rvc{{\mathbf{c}}}
\def\rvd{{\mathbf{d}}}
\def\rve{{\mathbf{e}}}
\def\rvf{{\mathbf{f}}}
\def\rvg{{\mathbf{g}}}
\def\rvh{{\mathbf{h}}}
\def\rvu{{\mathbf{i}}}
\def\rvj{{\mathbf{j}}}
\def\rvk{{\mathbf{k}}}
\def\rvl{{\mathbf{l}}}
\def\rvm{{\mathbf{m}}}
\def\rvn{{\mathbf{n}}}
\def\rvo{{\mathbf{o}}}
\def\rvp{{\mathbf{p}}}
\def\rvq{{\mathbf{q}}}
\def\rvr{{\mathbf{r}}}
\def\rvs{{\mathbf{s}}}
\def\rvt{{\mathbf{t}}}
\def\rvu{{\mathbf{u}}}
\def\rvv{{\mathbf{v}}}
\def\rvw{{\mathbf{w}}}
\def\rvx{{\mathbf{x}}}
\def\rvy{{\mathbf{y}}}
\def\rvz{{\mathbf{z}}}

% Elements of random vectors
\def\erva{{\textnormal{a}}}
\def\ervb{{\textnormal{b}}}
\def\ervc{{\textnormal{c}}}
\def\ervd{{\textnormal{d}}}
\def\erve{{\textnormal{e}}}
\def\ervf{{\textnormal{f}}}
\def\ervg{{\textnormal{g}}}
\def\ervh{{\textnormal{h}}}
\def\ervi{{\textnormal{i}}}
\def\ervj{{\textnormal{j}}}
\def\ervk{{\textnormal{k}}}
\def\ervl{{\textnormal{l}}}
\def\ervm{{\textnormal{m}}}
\def\ervn{{\textnormal{n}}}
\def\ervo{{\textnormal{o}}}
\def\ervp{{\textnormal{p}}}
\def\ervq{{\textnormal{q}}}
\def\ervr{{\textnormal{r}}}
\def\ervs{{\textnormal{s}}}
\def\ervt{{\textnormal{t}}}
\def\ervu{{\textnormal{u}}}
\def\ervv{{\textnormal{v}}}
\def\ervw{{\textnormal{w}}}
\def\ervx{{\textnormal{x}}}
\def\ervy{{\textnormal{y}}}
\def\ervz{{\textnormal{z}}}

% Random matrices
\def\rmA{{\mathbf{A}}}
\def\rmB{{\mathbf{B}}}
\def\rmC{{\mathbf{C}}}
\def\rmD{{\mathbf{D}}}
\def\rmE{{\mathbf{E}}}
\def\rmF{{\mathbf{F}}}
\def\rmG{{\mathbf{G}}}
\def\rmH{{\mathbf{H}}}
\def\rmI{{\mathbf{I}}}
\def\rmJ{{\mathbf{J}}}
\def\rmK{{\mathbf{K}}}
\def\rmL{{\mathbf{L}}}
\def\rmM{{\mathbf{M}}}
\def\rmN{{\mathbf{N}}}
\def\rmO{{\mathbf{O}}}
\def\rmP{{\mathbf{P}}}
\def\rmQ{{\mathbf{Q}}}
\def\rmR{{\mathbf{R}}}
\def\rmS{{\mathbf{S}}}
\def\rmT{{\mathbf{T}}}
\def\rmU{{\mathbf{U}}}
\def\rmV{{\mathbf{V}}}
\def\rmW{{\mathbf{W}}}
\def\rmX{{\mathbf{X}}}
\def\rmY{{\mathbf{Y}}}
\def\rmZ{{\mathbf{Z}}}

% Elements of random matrices
\def\ermA{{\textnormal{A}}}
\def\ermB{{\textnormal{B}}}
\def\ermC{{\textnormal{C}}}
\def\ermD{{\textnormal{D}}}
\def\ermE{{\textnormal{E}}}
\def\ermF{{\textnormal{F}}}
\def\ermG{{\textnormal{G}}}
\def\ermH{{\textnormal{H}}}
\def\ermI{{\textnormal{I}}}
\def\ermJ{{\textnormal{J}}}
\def\ermK{{\textnormal{K}}}
\def\ermL{{\textnormal{L}}}
\def\ermM{{\textnormal{M}}}
\def\ermN{{\textnormal{N}}}
\def\ermO{{\textnormal{O}}}
\def\ermP{{\textnormal{P}}}
\def\ermQ{{\textnormal{Q}}}
\def\ermR{{\textnormal{R}}}
\def\ermS{{\textnormal{S}}}
\def\ermT{{\textnormal{T}}}
\def\ermU{{\textnormal{U}}}
\def\ermV{{\textnormal{V}}}
\def\ermW{{\textnormal{W}}}
\def\ermX{{\textnormal{X}}}
\def\ermY{{\textnormal{Y}}}
\def\ermZ{{\textnormal{Z}}}

% Vectors
\def\vzero{{\bm{0}}}
\def\vone{{\bm{1}}}
\def\vmu{{\bm{\mu}}}
\def\vtheta{{\bm{\theta}}}
\def\va{{\bm{a}}}
\def\vb{{\bm{b}}}
\def\vc{{\bm{c}}}
\def\vd{{\bm{d}}}
\def\ve{{\bm{e}}}
\def\vf{{\bm{f}}}
\def\vg{{\bm{g}}}
\def\vh{{\bm{h}}}
\def\vi{{\bm{i}}}
\def\vj{{\bm{j}}}
\def\vk{{\bm{k}}}
\def\vl{{\bm{l}}}
\def\vm{{\bm{m}}}
\def\vn{{\bm{n}}}
\def\vo{{\bm{o}}}
\def\vp{{\bm{p}}}
\def\vq{{\bm{q}}}
\def\vr{{\bm{r}}}
\def\vs{{\bm{s}}}
\def\vt{{\bm{t}}}
\def\vu{{\bm{u}}}
\def\vv{{\bm{v}}}
\def\vw{{\bm{w}}}
\def\vx{{\bm{x}}}
\def\vy{{\bm{y}}}
\def\vz{{\bm{z}}}

% Elements of vectors
\def\evalpha{{\alpha}}
\def\evbeta{{\beta}}
\def\evepsilon{{\epsilon}}
\def\evlambda{{\lambda}}
\def\evomega{{\omega}}
\def\evmu{{\mu}}
\def\evpsi{{\psi}}
\def\evsigma{{\sigma}}
\def\evtheta{{\theta}}
\def\eva{{a}}
\def\evb{{b}}
\def\evc{{c}}
\def\evd{{d}}
\def\eve{{e}}
\def\evf{{f}}
\def\evg{{g}}
\def\evh{{h}}
\def\evi{{i}}
\def\evj{{j}}
\def\evk{{k}}
\def\evl{{l}}
\def\evm{{m}}
\def\evn{{n}}
\def\evo{{o}}
\def\evp{{p}}
\def\evq{{q}}
\def\evr{{r}}
\def\evs{{s}}
\def\evt{{t}}
\def\evu{{u}}
\def\evv{{v}}
\def\evw{{w}}
\def\evx{{x}}
\def\evy{{y}}
\def\evz{{z}}

% Matrix
\def\mA{{\bm{A}}}
\def\mB{{\bm{B}}}
\def\mC{{\bm{C}}}
\def\mD{{\bm{D}}}
\def\mE{{\bm{E}}}
\def\mF{{\bm{F}}}
\def\mG{{\bm{G}}}
\def\mH{{\bm{H}}}
\def\mI{{\bm{I}}}
\def\mJ{{\bm{J}}}
\def\mK{{\bm{K}}}
\def\mL{{\bm{L}}}
\def\mM{{\bm{M}}}
\def\mN{{\bm{N}}}
\def\mO{{\bm{O}}}
\def\mP{{\bm{P}}}
\def\mQ{{\bm{Q}}}
\def\mR{{\bm{R}}}
\def\mS{{\bm{S}}}
\def\mT{{\bm{T}}}
\def\mU{{\bm{U}}}
\def\mV{{\bm{V}}}
\def\mW{{\bm{W}}}
\def\mX{{\bm{X}}}
\def\mY{{\bm{Y}}}
\def\mZ{{\bm{Z}}}
\def\mBeta{{\bm{\beta}}}
\def\mPhi{{\bm{\Phi}}}
\def\mLambda{{\bm{\Lambda}}}
\def\mSigma{{\bm{\Sigma}}}

% Tensor
\DeclareMathAlphabet{\mathsfit}{\encodingdefault}{\sfdefault}{m}{sl}
\SetMathAlphabet{\mathsfit}{bold}{\encodingdefault}{\sfdefault}{bx}{n}
\newcommand{\tens}[1]{\bm{\mathsfit{#1}}}
\def\tA{{\tens{A}}}
\def\tB{{\tens{B}}}
\def\tC{{\tens{C}}}
\def\tD{{\tens{D}}}
\def\tE{{\tens{E}}}
\def\tF{{\tens{F}}}
\def\tG{{\tens{G}}}
\def\tH{{\tens{H}}}
\def\tI{{\tens{I}}}
\def\tJ{{\tens{J}}}
\def\tK{{\tens{K}}}
\def\tL{{\tens{L}}}
\def\tM{{\tens{M}}}
\def\tN{{\tens{N}}}
\def\tO{{\tens{O}}}
\def\tP{{\tens{P}}}
\def\tQ{{\tens{Q}}}
\def\tR{{\tens{R}}}
\def\tS{{\tens{S}}}
\def\tT{{\tens{T}}}
\def\tU{{\tens{U}}}
\def\tV{{\tens{V}}}
\def\tW{{\tens{W}}}
\def\tX{{\tens{X}}}
\def\tY{{\tens{Y}}}
\def\tZ{{\tens{Z}}}


% Graph
\def\gA{{\mathcal{A}}}
\def\gB{{\mathcal{B}}}
\def\gC{{\mathcal{C}}}
\def\gD{{\mathcal{D}}}
\def\gE{{\mathcal{E}}}
\def\gF{{\mathcal{F}}}
\def\gG{{\mathcal{G}}}
\def\gH{{\mathcal{H}}}
\def\gI{{\mathcal{I}}}
\def\gJ{{\mathcal{J}}}
\def\gK{{\mathcal{K}}}
\def\gL{{\mathcal{L}}}
\def\gM{{\mathcal{M}}}
\def\gN{{\mathcal{N}}}
\def\gO{{\mathcal{O}}}
\def\gP{{\mathcal{P}}}
\def\gQ{{\mathcal{Q}}}
\def\gR{{\mathcal{R}}}
\def\gS{{\mathcal{S}}}
\def\gT{{\mathcal{T}}}
\def\gU{{\mathcal{U}}}
\def\gV{{\mathcal{V}}}
\def\gW{{\mathcal{W}}}
\def\gX{{\mathcal{X}}}
\def\gY{{\mathcal{Y}}}
\def\gZ{{\mathcal{Z}}}

% Sets
\def\sA{{\mathbb{A}}}
\def\sB{{\mathbb{B}}}
\def\sC{{\mathbb{C}}}
\def\sD{{\mathbb{D}}}
% Don't use a set called E, because this would be the same as our symbol
% for expectation.
\def\sF{{\mathbb{F}}}
\def\sG{{\mathbb{G}}}
\def\sH{{\mathbb{H}}}
\def\sI{{\mathbb{I}}}
\def\sJ{{\mathbb{J}}}
\def\sK{{\mathbb{K}}}
\def\sL{{\mathbb{L}}}
\def\sM{{\mathbb{M}}}
\def\sN{{\mathbb{N}}}
\def\sO{{\mathbb{O}}}
\def\sP{{\mathbb{P}}}
\def\sQ{{\mathbb{Q}}}
\def\sR{{\mathbb{R}}}
\def\sS{{\mathbb{S}}}
\def\sT{{\mathbb{T}}}
\def\sU{{\mathbb{U}}}
\def\sV{{\mathbb{V}}}
\def\sW{{\mathbb{W}}}
\def\sX{{\mathbb{X}}}
\def\sY{{\mathbb{Y}}}
\def\sZ{{\mathbb{Z}}}

% Entries of a matrix
\def\emLambda{{\Lambda}}
\def\emA{{A}}
\def\emB{{B}}
\def\emC{{C}}
\def\emD{{D}}
\def\emE{{E}}
\def\emF{{F}}
\def\emG{{G}}
\def\emH{{H}}
\def\emI{{I}}
\def\emJ{{J}}
\def\emK{{K}}
\def\emL{{L}}
\def\emM{{M}}
\def\emN{{N}}
\def\emO{{O}}
\def\emP{{P}}
\def\emQ{{Q}}
\def\emR{{R}}
\def\emS{{S}}
\def\emT{{T}}
\def\emU{{U}}
\def\emV{{V}}
\def\emW{{W}}
\def\emX{{X}}
\def\emY{{Y}}
\def\emZ{{Z}}
\def\emSigma{{\Sigma}}

% entries of a tensor
% Same font as tensor, without \bm wrapper
\newcommand{\etens}[1]{\mathsfit{#1}}
\def\etLambda{{\etens{\Lambda}}}
\def\etA{{\etens{A}}}
\def\etB{{\etens{B}}}
\def\etC{{\etens{C}}}
\def\etD{{\etens{D}}}
\def\etE{{\etens{E}}}
\def\etF{{\etens{F}}}
\def\etG{{\etens{G}}}
\def\etH{{\etens{H}}}
\def\etI{{\etens{I}}}
\def\etJ{{\etens{J}}}
\def\etK{{\etens{K}}}
\def\etL{{\etens{L}}}
\def\etM{{\etens{M}}}
\def\etN{{\etens{N}}}
\def\etO{{\etens{O}}}
\def\etP{{\etens{P}}}
\def\etQ{{\etens{Q}}}
\def\etR{{\etens{R}}}
\def\etS{{\etens{S}}}
\def\etT{{\etens{T}}}
\def\etU{{\etens{U}}}
\def\etV{{\etens{V}}}
\def\etW{{\etens{W}}}
\def\etX{{\etens{X}}}
\def\etY{{\etens{Y}}}
\def\etZ{{\etens{Z}}}

% The true underlying data generating distribution
\newcommand{\pdata}{p_{\rm{data}}}
% The empirical distribution defined by the training set
\newcommand{\ptrain}{\hat{p}_{\rm{data}}}
\newcommand{\Ptrain}{\hat{P}_{\rm{data}}}
% The model distribution
\newcommand{\pmodel}{p_{\rm{model}}}
\newcommand{\Pmodel}{P_{\rm{model}}}
\newcommand{\ptildemodel}{\tilde{p}_{\rm{model}}}
% Stochastic autoencoder distributions
\newcommand{\pencode}{p_{\rm{encoder}}}
\newcommand{\pdecode}{p_{\rm{decoder}}}
\newcommand{\precons}{p_{\rm{reconstruct}}}

\newcommand{\laplace}{\mathrm{Laplace}} % Laplace distribution

\newcommand{\E}{\mathbb{E}}
\newcommand{\Ls}{\mathcal{L}}
\newcommand{\R}{\mathbb{R}}
\newcommand{\emp}{\tilde{p}}
\newcommand{\lr}{\alpha}
\newcommand{\reg}{\lambda}
\newcommand{\rect}{\mathrm{rectifier}}
\newcommand{\softmax}{\mathrm{softmax}}
\newcommand{\sigmoid}{\sigma}
\newcommand{\softplus}{\zeta}
\newcommand{\KL}{D_{\mathrm{KL}}}
\newcommand{\Var}{\mathrm{Var}}
\newcommand{\standarderror}{\mathrm{SE}}
\newcommand{\Cov}{\mathrm{Cov}}
% Wolfram Mathworld says $L^2$ is for function spaces and $\ell^2$ is for vectors
% But then they seem to use $L^2$ for vectors throughout the site, and so does
% wikipedia.
\newcommand{\normlzero}{L^0}
\newcommand{\normlone}{L^1}
\newcommand{\normltwo}{L^2}
\newcommand{\normlp}{L^p}
\newcommand{\normmax}{L^\infty}

\newcommand{\parents}{Pa} % See usage in notation.tex. Chosen to match Daphne's book.

\DeclareMathOperator*{\argmax}{arg\,max}
\DeclareMathOperator*{\argmin}{arg\,min}

\DeclareMathOperator{\sign}{sign}
\DeclareMathOperator{\Tr}{Tr}
\let\ab\allowbreak


==> sec/checklist.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\section*{Checklist}

%%% BEGIN INSTRUCTIONS %%%
The checklist follows the references.  Please
read the checklist guidelines carefully for information on how to answer these
questions.  For each question, change the default \answerTODO{} to \answerYes{},
\answerNo{}, or \answerNA{}.  You are strongly encouraged to include a {\bf
justification to your answer}, either by referencing the appropriate section of
your paper or providing a brief inline description.  For example:
\begin{itemize}
  \item Did you include the license to the code and datasets? \answerYes{See Section 3.}
  \item Did you include the license to the code and datasets? \answerNo{The code and the data are proprietary.}
  \item Did you include the license to the code and datasets? \answerNA{}
\end{itemize}
Please do not modify the questions and only use the provided macros for your
answers.  Note that the Checklist section does not count towards the page
limit.  In your paper, please delete this instructions block and only keep the
Checklist section heading above along with the questions/answers below.
%%% END INSTRUCTIONS %%%

\begin{enumerate}

\item For all authors...
\begin{enumerate}
  \item Do the main claims made in the abstract and introduction accurately reflect the paper's contributions and scope?
    \answerYes{}
  \item Did you describe the limitations of your work?
    \answerYes{}
  \item Did you discuss any potential negative societal impacts of your work?
    \answerYes{}
  \item Have you read the ethics review guidelines and ensured that your paper conforms to them?
    \answerYes{}
\end{enumerate}

\item If you are including theoretical results...
\begin{enumerate}
  \item Did you state the full set of assumptions of all theoretical results?
    \answerNA{}
	\item Did you include complete proofs of all theoretical results?
  \answerNA{}
\end{enumerate}

\item If you ran experiments (e.g. for benchmarks)...
\begin{enumerate}
  \item Did you include the code, data, and instructions needed to reproduce the main experimental results (either in the supplemental material or as a URL)?
    \answerYes{We will release the code and data. For details needed to reproduce our work, see \autoref{sec:benchmark} and \autoref{sec:llm-crowd-details}.}
  \item Did you specify all the training details (e.g., data splits, hyperparameters, how they were chosen)?
    \answerNA{} Our baselines are established via querying existing models via APIs. This involves no training. We make no attempt to fine-tune any model in this work.
	\item Did you report error bars (e.g., with respect to the random seed after running experiments multiple times)?
    \answerYes{See \autoref{sec:llm-crowd-details}.}
	\item Did you include the total amount of compute and the type of resources used (e.g., type of GPUs, internal cluster, or cloud provider)?
    \answerNA{}
\end{enumerate}

\item If you are using existing assets (e.g., code, data, models) or curating/releasing new assets...
\begin{enumerate}
  \item If your work uses existing assets, did you cite the creators?
    \answerYes{}
  \item Did you mention the license of the assets?
    \answerYes{} See \autoref{table:question_bank_licenses} in \autoref{subsection:dataset_licenses}
  \item Did you include any new assets either in the supplemental material or as a URL?
    \answerYes{}
  \item Did you discuss whether and how consent was obtained from people whose data you're using/curating?
    \answerYes{} See \autoref{sec:human} discussion on IRB approval
  \item Did you discuss whether the data you are using/curating contains personally identifiable information or offensive content?
    \answerYes{} See \autoref{sec:human}  
\end{enumerate}

\item If you used crowdsourcing or conducted research with human subjects...
\begin{enumerate}
  \item Did you include the full text of instructions given to participants and screenshots, if applicable?
    \answerYes{} See \autoref{appendix:human_survey}
  \item Did you describe any potential participant risks, with links to Institutional Review Board (IRB) approvals, if applicable?
    \answerYes{} See \autoref{sec:human}. We cannot provide a link to the IRB approval without leaking author information; however, the protocol number we're working with is 855431.
  \item Did you include the estimated hourly wage paid to participants and the total amount spent on participant compensation?
    \answerYes{} See \autoref{sec:human}
\end{enumerate}

\end{enumerate}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

==> tables/combined_leaderboard.tex <==
\begin{table}[ht!]
\caption{Leaderboard with Top 10 Models}
\label{table:combined_leaderboard}
\centering
\resizebox{\textwidth}{!} {%
\Large
\begin{tabular}{@{}l l l l >{\centering\arraybackslash}m{2cm} >{\centering\arraybackslash}m{2cm} >{\centering\arraybackslash}m{2cm} >{\centering\arraybackslash}m{3cm} >{\centering\arraybackslash}m{2cm} >{\centering\arraybackslash}m{2cm}@{}}
\toprule
\multicolumn{10}{c}{\textbf{Panel A: Includes human comparison group and evaluates the set of 200 questions received by humans}} \\ \addlinespace
& & & & \multicolumn{3}{c}{Brier Score $\downarrow$} \\ \cmidrule(lr){5-7}
Model & Organization & \begin{tabular}[c]{@{}l@{}}Information\\ provided\end{tabular} & Prompt & \begin{tabular}[c]{@{}l@{}}Dataset\\(N=316)\end{tabular} & \begin{tabular}[c]{@{}l@{}}Market\\(N=77)\end{tabular} & \begin{tabular}[c]{@{}l@{}}Overall\\(N=393)\end{tabular} & \begin{tabular}[c]{@{}l@{}}Confidence\\ Interval\end{tabular} & \begin{tabular}[c]{@{}l@{}}Pairwise\\p-value\\comparing\\to No. 1\end{tabular} & \begin{tabular}[c]{@{}l@{}}Pct. more \\accurate\\ than No. 1\end{tabular} \\
\midrule
Superforecaster median forecast & ForecastBench & -- & -- & 0.126 & 0.056 & 0.091 & [0.072, 0.110] & -- & 0\% \\
Claude-3-5-Sonnet-20240620 & Anthropic & Freeze values & Scratchpad & 0.140 & 0.082 & 0.111 & [0.090, 0.132] & 0.001 & 33\% \\
Public median forecast & ForecastBench & -- & -- & 0.156 & 0.066 & 0.111 & [0.093, 0.129] & <0.001 & 25\% \\
Claude-3-5-Sonnet-20240620 & Anthropic & News with freeze values & Scratchpad & 0.144 & 0.087 & 0.116 & [0.095, 0.137] & <0.001 & 30\% \\
Claude-3-5-Sonnet-20240620 & Anthropic & Freeze values & Zero shot & 0.145 & 0.092 & 0.118 & [0.092, 0.144] & <0.001 & 33\% \\
GPT-4 & OpenAI & Freeze values & Zero shot & 0.165 & 0.072 & 0.118 & [0.098, 0.139] & <0.001 & 33\% \\
GPT-4-Turbo-2024-04-09 & OpenAI & Freeze values & Zero shot & 0.171 & 0.071 & 0.121 & [0.100, 0.141] & <0.001 & 34\% \\
GPT-4o & OpenAI & News with freeze values & Scratchpad & 0.169 & 0.076 & 0.122 & [0.105, 0.140] & <0.001 & 26\% \\
Claude-3-5-Sonnet-20240620 & Anthropic & -- & Scratchpad & 0.140 & 0.110 & 0.125 & [0.103, 0.146] & <0.001 & 28\% \\
GPT-4o & OpenAI & Freeze values & Scratchpad & 0.164 & 0.087 & 0.125 & [0.106, 0.144] & <0.001 & 27\% \\
Always 0.5 & ForecastBench & -- & -- & 0.250 & 0.076 & 0.163 & [0.149, 0.177] & <0.001 & 28\% \\
\midrule
\multicolumn{10}{c}{\textbf{Panel B: Excludes human comparison group and evaluates the set of 1,000 questions received by LLMs}} \\ \addlinespace
& & & & \multicolumn{3}{c}{Brier Score $\downarrow$} \\ \cmidrule(lr){5-7}
Model & Organization & \begin{tabular}[c]{@{}l@{}}Information\\ provided\end{tabular} & Prompt & \begin{tabular}[c]{@{}l@{}}Dataset\\(N=4,107)\end{tabular} & \begin{tabular}[c]{@{}l@{}}Market\\(N=907)\end{tabular} & \begin{tabular}[c]{@{}l@{}}Overall\\(N=5,014)\end{tabular} & \begin{tabular}[c]{@{}l@{}}Confidence\\ Interval\end{tabular} & \begin{tabular}[c]{@{}l@{}}Pairwise\\p-value\\comparing\\to No. 1\end{tabular} & \begin{tabular}[c]{@{}l@{}}Pct. more \\accurate\\ than No. 1\end{tabular} \\
\midrule
Claude-3-5-Sonnet-20240620 & Anthropic & Freeze values & Scratchpad & 0.170 & 0.059 & 0.115 & [0.109, 0.121] & -- & 0\% \\
GPT-4-Turbo-2024-04-09 & OpenAI & Freeze values & Scratchpad & 0.171 & 0.063 & 0.117 & [0.111, 0.122] & 0.168 & 42\% \\
GPT-4o & OpenAI & Freeze values & Scratchpad & 0.191 & 0.052 & 0.122 & [0.117, 0.127] & <0.001 & 43\% \\
Gemini-1.5-Pro & Google & Freeze values & Scratchpad & 0.162 & 0.087 & 0.125 & [0.119, 0.130] & <0.001 & 34\% \\
GPT-4o & OpenAI & News with freeze values & Scratchpad & 0.192 & 0.064 & 0.128 & [0.122, 0.133] & <0.001 & 39\% \\
Gemini-1.5-Pro & Google & News with freeze values & Scratchpad & 0.167 & 0.092 & 0.130 & [0.124, 0.135] & <0.001 & 34\% \\
Claude-3-Opus-20240229 & Anthropic & Freeze values & Zero shot & 0.190 & 0.073 & 0.131 & [0.125, 0.137] & <0.001 & 41\% \\
Qwen1.5-110B-Chat & Qwen & Freeze values & Scratchpad & 0.176 & 0.090 & 0.133 & [0.128, 0.139] & <0.001 & 30\% \\
GPT-4-Turbo-2024-04-09 & OpenAI & -- & Scratchpad & 0.171 & 0.096 & 0.133 & [0.128, 0.139] & <0.001 & 30\% \\
Claude-3-5-Sonnet-20240620 & Anthropic & News with freeze values & Scratchpad & 0.187 & 0.080 & 0.134 & [0.128, 0.139] & <0.001 & 31\% \\
Always 0.5 & ForecastBench & -- & -- & 0.250 & 0.051 & 0.150 & [0.147, 0.154] & <0.001 & 46\% \\
\bottomrule
\end{tabular}
}
\begin{minipage}{\textwidth} 
{\tiny
    \textit{Notes:} \\
    \vspace{-2mm} 
    \refereeresponse{1. The leaderboard evaluates performance at the 7-, 30-, and 90-day forecast horizons.}\\
    \vspace{-2mm} 
    \refereeresponse{2. Panel A shows performance on the 200 standard questions provided in the human question set. Panel B shows performance on the 1,000 (500 standard, 500}\\
    \vspace{-2mm}
    \refereeresponse{combination) questions in the LLM question set.}\\
    \vspace{-2mm}
    3. We only show the performance of one model from each model series. The full leaderboard is available at \href{\BenchmarkURL}{\BenchmarkURL}. Online results are updated nightly, \vspace{-2mm} so may be slightly different than the static version presented here.\\
    \vspace{-2mm} % reduces space between this line and the next one
    4. For resolved questions, predictions are compared against ground truth, while for unresolved questions, predictions are compared to community aggregates.\\
    \vspace{-2mm} % reduces space between this line and the next one
    5. The overall score is calculated as the average of the mean dataset Brier score and the mean market Brier score.\\
    \vspace{-2mm} % reduces space between this line and the next one
    6. Pct. more accurate than No. 1: The percent of questions where this forecaster had a better overall score than the best forecaster (with rank 1).\\
    \vspace{-2mm} % reduces space between this line and the next one
    7. Pairwise p-value comparing to No. 1 (bootstrapped): The p-value calculated by bootstrapping the differences in overall score between each model and the best forecaster (the group with rank 1) under the null hypothesis that there's no difference.
}
\end{minipage}

\end{table}


==> tables/human_combo_generated_leaderboard_overall.tex <==
\begin{table}[ht!]
\caption{Leaderboard with Performance on Combination Questions (Independence): Top 50}
\label{table:human_llm_combo_generated_top_50}
\centering
\resizebox{\textwidth}{!} {
\Large
\begin{tabular}{@{}l l l l >{\centering\arraybackslash}m{2cm} >{\centering\arraybackslash}m{2cm} >{\centering\arraybackslash}m{2cm} >{\centering\arraybackslash}m{3cm} >{\centering\arraybackslash}m{2cm} >{\centering\arraybackslash}m{2cm}@{}}
\toprule
& & & & \multicolumn{3}{c}{Brier Score $\downarrow$} \\ \cmidrule(lr){5-7}
Model & Organization & \begin{tabular}[c]{@{}l@{}}Information\\ provided\end{tabular} & Prompt & \begin{tabular}[c]{@{}l@{}}Dataset\\(N=870)\end{tabular} & \begin{tabular}[c]{@{}l@{}}Market\\(N=301)\end{tabular} & \begin{tabular}[c]{@{}l@{}}Overall\\(N=1,171)\end{tabular} & \begin{tabular}[c]{@{}l@{}}Confidence\\ Interval\end{tabular} & \begin{tabular}[c]{@{}l@{}}Pairwise\\p-value\\comparing\\to No. 1\end{tabular} & \begin{tabular}[c]{@{}l@{}}Pct. more \\accurate\\ than No. 1\end{tabular} \\
\midrule
Superforecaster median forecast & ForecastBench & -- & -- & 0.097 & 0.04 & 0.068 & [0.06, 0.077] & -- & 0\% \\
Public median forecast & ForecastBench & -- & -- & 0.127 & 0.039 & 0.083 & [0.075, 0.091] & $<$0.001 & 28\% \\
GPT-4 & OpenAI & Freeze values & Zero shot & 0.131 & 0.041 & 0.086 & [0.077, 0.095] & $<$0.001 & 34\% \\
GPT-4-Turbo-2024-04-09 & OpenAI & Freeze values & Zero shot & 0.135 & 0.04 & 0.088 & [0.079, 0.097] & $<$0.001 & 33\% \\
Claude-3-5-Sonnet-20240620 & Anthropic & Freeze values & Zero shot & 0.114 & 0.062 & 0.088 & [0.076, 0.1] & $<$0.001 & 34\% \\
Claude-3-5-Sonnet-20240620 & Anthropic & Freeze values & Scratchpad & 0.118 & 0.064 & 0.091 & [0.08, 0.102] & $<$0.001 & 28\% \\
GPT-4o & OpenAI & Freeze values & Scratchpad & 0.134 & 0.052 & 0.093 & [0.084, 0.102] & $<$0.001 & 28\% \\
Claude-3-5-Sonnet-20240620 & Anthropic & News with freeze values & Scratchpad & 0.13 & 0.06 & 0.095 & [0.085, 0.105] & $<$0.001 & 28\% \\
GPT-4o & OpenAI & News with freeze values & Scratchpad & 0.142 & 0.049 & 0.096 & [0.087, 0.104] & $<$0.001 & 27\% \\
Mistral-Large-Latest & Mistral AI & Freeze values & Zero shot & 0.134 & 0.062 & 0.098 & [0.088, 0.108] & $<$0.001 & 25\% \\
Mistral-Large-Latest & Mistral AI & Freeze values & Scratchpad & 0.13 & 0.068 & 0.099 & [0.091, 0.107] & $<$0.001 & 24\% \\
Claude-3-Opus-20240229 & Anthropic & Freeze values & Zero shot & 0.146 & 0.057 & 0.102 & [0.091, 0.112] & $<$0.001 & 30\% \\
Claude-3-5-Sonnet-20240620 & Anthropic & No & Scratchpad & 0.118 & 0.086 & 0.102 & [0.09, 0.113] & $<$0.001 & 26\% \\
Claude-2.1 & Anthropic & Freeze values & Scratchpad & 0.163 & 0.042 & 0.102 & [0.095, 0.11] & $<$0.001 & 29\% \\
Llama-3-70b-Chat-Hf & Meta & Freeze values & Zero shot & 0.139 & 0.067 & 0.103 & [0.093, 0.114] & $<$0.001 & 26\% \\
GPT-4o & OpenAI & No & Scratchpad & 0.134 & 0.073 & 0.104 & [0.094, 0.113] & $<$0.001 & 24\% \\
Claude-3-5-Sonnet-20240620 & Anthropic & News & No & 0.135 & 0.074 & 0.104 & [0.094, 0.114] & $<$0.001 & 25\% \\
Qwen1.5-110B-Chat & Qwen & Freeze values & Zero shot & 0.153 & 0.056 & 0.105 & [0.096, 0.114] & $<$0.001 & 26\% \\
Claude-3-Opus-20240229 & Anthropic & Freeze values & Scratchpad & 0.135 & 0.076 & 0.105 & [0.096, 0.115] & $<$0.001 & 24\% \\
GPT-4 & OpenAI & Freeze values & Scratchpad & 0.151 & 0.061 & 0.106 & [0.097, 0.114] & $<$0.001 & 24\% \\
Claude-3-5-Sonnet-20240620 & Anthropic & News & Scratchpad & 0.13 & 0.083 & 0.107 & [0.096, 0.118] & $<$0.001 & 24\% \\
Claude-2.1 & Anthropic & No & Scratchpad & 0.163 & 0.052 & 0.107 & [0.099, 0.116] & $<$0.001 & 27\% \\
Claude-3-5-Sonnet-20240620 & Anthropic & No & Zero shot & 0.114 & 0.101 & 0.107 & [0.094, 0.12] & $<$0.001 & 26\% \\
Llama-3-70b-Chat-Hf & Meta & Freeze values & Scratchpad & 0.151 & 0.064 & 0.108 & [0.099, 0.116] & $<$0.001 & 23\% \\
Mixtral-8x22B-Instruct-V0.1 & Mistral AI & Freeze values & Zero shot & 0.154 & 0.066 & 0.11 & [0.099, 0.121] & $<$0.001 & 29\% \\
Gemini-1.5-Flash & Google & Freeze values & Scratchpad & 0.151 & 0.069 & 0.11 & [0.1, 0.12] & $<$0.001 & 25\% \\
Claude-3-5-Sonnet-20240620 & Anthropic & News & No & 0.136 & 0.085 & 0.11 & [0.099, 0.121] & $<$0.001 & 24\% \\
GPT-4o & OpenAI & Freeze values & Zero shot & 0.166 & 0.055 & 0.11 & [0.1, 0.121] & $<$0.001 & 30\% \\
GPT-4o & OpenAI & News & Scratchpad & 0.142 & 0.08 & 0.111 & [0.1, 0.122] & $<$0.001 & 23\% \\
Gemini-1.5-Pro & Google & Freeze values & Zero shot & 0.154 & 0.068 & 0.111 & [0.099, 0.123] & $<$0.001 & 28\% \\
Gemini-1.5-Pro & Google & Freeze values & Scratchpad & 0.139 & 0.084 & 0.111 & [0.102, 0.121] & $<$0.001 & 23\% \\
Claude-3-Opus-20240229 & Anthropic & No & Scratchpad & 0.135 & 0.088 & 0.111 & [0.102, 0.121] & $<$0.001 & 23\% \\
GPT-4-Turbo-2024-04-09 & OpenAI & Freeze values & Scratchpad & 0.152 & 0.072 & 0.112 & [0.101, 0.122] & $<$0.001 & 26\% \\
GPT-4-Turbo-2024-04-09 & OpenAI & No & Zero shot & 0.135 & 0.089 & 0.112 & [0.102, 0.123] & $<$0.001 & 22\% \\
GPT-4 & OpenAI & No & Zero shot & 0.131 & 0.095 & 0.113 & [0.103, 0.122] & $<$0.001 & 24\% \\
Gemini-1.5-Pro & Google & News with freeze values & Scratchpad & 0.143 & 0.084 & 0.113 & [0.103, 0.123] & $<$0.001 & 22\% \\
Mistral-Large-Latest & Mistral AI & No & Scratchpad & 0.13 & 0.097 & 0.113 & [0.104, 0.123] & $<$0.001 & 23\% \\
Mixtral-8x22B-Instruct-V0.1 & Mistral AI & Freeze values & Scratchpad & 0.15 & 0.077 & 0.114 & [0.105, 0.123] & $<$0.001 & 23\% \\
Gemini-1.5-Flash & Google & Freeze values & Zero shot & 0.15 & 0.078 & 0.114 & [0.101, 0.127] & $<$0.001 & 27\% \\
Gemini-1.5-Pro & Google & No & Scratchpad & 0.139 & 0.09 & 0.115 & [0.105, 0.124] & $<$0.001 & 22\% \\
GPT-4 & OpenAI & No & Scratchpad & 0.151 & 0.079 & 0.115 & [0.106, 0.123] & $<$0.001 & 21\% \\
Imputed Forecaster & ForecastBench & -- & -- & 0.203 & 0.029 & 0.116 & [0.107, 0.124] & $<$0.001 & 32\% \\
Gemini-1.5-Pro & Google & News & Scratchpad & 0.143 & 0.091 & 0.117 & [0.107, 0.127] & $<$0.001 & 23\% \\
GPT-4-Turbo-2024-04-09 & OpenAI & No & Scratchpad & 0.152 & 0.082 & 0.117 & [0.108, 0.127] & $<$0.001 & 21\% \\
Claude-2.1 & Anthropic & Freeze values & Zero shot & 0.179 & 0.055 & 0.117 & [0.107, 0.127] & $<$0.001 & 29\% \\
GPT-4-Turbo-2024-04-09 & OpenAI & News with freeze values & Scratchpad & 0.161 & 0.075 & 0.118 & [0.108, 0.129] & $<$0.001 & 26\% \\
Claude-3-Opus-20240229 & Anthropic & No & Zero shot & 0.146 & 0.093 & 0.119 & [0.108, 0.131] & $<$0.001 & 24\% \\
Claude-3-Opus-20240229 & Anthropic & News & No & 0.134 & 0.106 & 0.12 & [0.11, 0.131] & $<$0.001 & 23\% \\
Llama-3-70b-Chat-Hf & Meta & No & Zero shot & 0.139 & 0.102 & 0.12 & [0.11, 0.131] & $<$0.001 & 23\% \\
Gemini-1.5-Flash & Google & No & Scratchpad & 0.151 & 0.09 & 0.12 & [0.11, 0.13] & $<$0.001 & 22\% \\
\bottomrule
\end{tabular}
}
\begin{minipage}{\textwidth} 
{\tiny
    \textit{Notes:} \\
    \vspace{-2mm} Pairwise p-value comparing to No. 1 (bootstrapped): The p-value calculated by bootstrapping the differences in overall score between each model and the best forecaster (the group with rank 1) under the null hypothesis that there's no difference.\\
    \vspace{-2mm} Pct. more accurate than No. 1: The percent of questions where this forecaster had a better overall score than the best forecaster (with rank 1).
}
\end{minipage}

\end{table}


==> tables/short_leaderboard.tex <==





\begin{table}[ht!]
    \caption{Benchmark performance by model. Includes human comparison group. Bold entry is the baseline naive forecast described in Section 3.4. Lower Brier Score is better. We will release an interactive website version with the full list of models.}
    \label{table:results}
    \centering
    \resizebox{\textwidth}{!} {%
      \large
      \begin{tabular}{@{}l l l l >{\centering\arraybackslash}m{2cm} >{\centering\arraybackslash}m{2cm} >{\centering\arraybackslash}m{3cm} >{\centering\arraybackslash}m{2cm}@{}}
        \toprule
        & & & & \multicolumn{3}{c}{Brier Score} & \\ \cmidrule(lr){5-7}
        Model & Organization & \begin{tabular}[c]{@{}l@{}}Information\\ provided\end{tabular} & Prompt & \multicolumn{1}{c}{Dataset} & \multicolumn{1}{c}{Market} & \multicolumn{1}{c}{Overall (2 Std Errors)} & \multicolumn{1}{c}{Z-score} \\ 
        \midrule
        \begin{tabular}[c]{@{}l@{}}Human median\end{tabular} & ForecastBench & --- & --- & 0.197 & 0.014 & 0.090 (0.025) & -0.003 \\
        \textbf{\begin{tabular}[c]{@{}l@{}}Naive forecast\end{tabular}} & \textbf{ForecastBench} & --- & --- & \textbf{0.209} & \textbf{0.006} & \textbf{0.090 (0.021)} & \textbf{0.000} \\
        GPT-4o & OpenAI & \begin{tabular}[c]{@{}l@{}}random set\end{tabular} & \begin{tabular}[c]{@{}l@{}}$\ddagger$\end{tabular} & 0.135 & 0.066 & 0.095 (0.018) & 0.028 \\
        \begin{tabular}[c]{@{}l@{}}Ensemble models$^\dagger$\end{tabular} & LLM Crowd & \begin{tabular}[c]{@{}l@{}}random set\end{tabular} & \begin{tabular}[c]{@{}l@{}}$\S$\end{tabular} & 0.157 & 0.068 & 0.105 (0.018) & 0.088 \\
        \begin{tabular}[c]{@{}l@{}}GPT-4o\end{tabular} & OpenAI & \begin{tabular}[c]{@{}l@{}}Yes\end{tabular} & scratchpad & 0.171 & 0.068 & 0.111 (0.025) & 0.124 \\
        \begin{tabular}[c]{@{}l@{}}Qwen1.5-110B-Chat\end{tabular} & Qwen & \begin{tabular}[c]{@{}l@{}}random set \end{tabular} & \begin{tabular}[c]{@{}l@{}}$\ddagger$\end{tabular} & 0.158 & 0.081 & 0.113 (0.019) & 0.137 \\
        \begin{tabular}[c]{@{}l@{}}GPT-4o\end{tabular} & OpenAI & No & zero-shot & 0.185 & 0.072 & 0.119 (0.030) & 0.172 \\
        \begin{tabular}[c]{@{}l@{}}GPT-4\end{tabular} & OpenAI & No & scratchpad & 0.175 & 0.080 & 0.119 (0.021) & 0.174 \\
        \begin{tabular}[c]{@{}l@{}}Claude-2.1\end{tabular} & Anthropic & No & scratchpad & 0.228 & 0.043 & 0.119 (0.018) & 0.176 \\
        \begin{tabular}[c]{@{}l@{}}GPT-4o\end{tabular} & OpenAI & No & scratchpad & 0.191 & 0.076 & 0.124 (0.029) & 0.200 \\
        \begin{tabular}[c]{@{}l@{}}Mistral-Large-Latest\end{tabular} & Mistral AI & No & scratchpad & 0.173 & 0.090 & 0.124 (0.022) & 0.204 \\
        \begin{tabular}[c]{@{}l@{}}Claude-3-Haiku-20240307\end{tabular} & Anthropic & No & zero-shot & 0.240 & 0.081 & 0.147 (0.015) & 0.339 \\
        Always 0.5 & ForecastBench & --- & --- & 0.250 & 0.119 & 0.173 (0.012) & 0.494 \\ \bottomrule
    \end{tabular}
    }
    {\raggedright\scriptsize\(\dagger\) Median of GPT-4o, Mistral-Large, and Qwen-1.5-110B (see details at Section 3.4)\\
    \(\ddagger\) Superforecaster prompt 3 (see Figure 12)\\\(\S\) All superforecaster prompts (see Figures 10, 11, and 12)\\
    See full leaderboard using the anonymized URL link: \url{https://storage.googleapis.com/30e089eb5ad0cff1702d4a5776cc90f3_pub/lm_human_leaderboard_overall.html}.\\
    The z-score reported is relative to the `naive' mean, a representation of one's performance if they forecasted the status quo for all questions; this is because the `naive' mean serves as a control, unaffected by the researchers' decisions around noise and variance.\\
    }
\end{table}

==> tables/short_leaderboard_nonhuman.tex <==

\begin{table}[ht!]
    \caption{Benchmark performance by model. Excludes human comparison group, contains questions humans did not forecast. Bold entry is the baseline naive forecast described in Section 3.4. Lower Brier Score is better. We will release an interactive website version with the full list of models.}
    \label{table:results_nonhuman}
    \centering
    \resizebox{\textwidth}{!} {%
      \large
      \begin{tabular}{@{}l l l l >{\centering\arraybackslash}m{2cm} >{\centering\arraybackslash}m{2cm} >{\centering\arraybackslash}m{3cm} >{\centering\arraybackslash}m{2cm}@{}}
        \toprule
        & & & & \multicolumn{3}{c}{Brier Score} & \\ \cmidrule(lr){5-7}
        Model & Organization & \begin{tabular}[c]{@{}l@{}}Information\\ provided\end{tabular} & Prompt & \multicolumn{1}{c}{Dataset} & \multicolumn{1}{c}{Market} & \multicolumn{1}{c}{Overall (2 Std Errors)} & \multicolumn{1}{c}{Z-score} \\ 
        \midrule
        \textbf{\begin{tabular}[c]{@{}l@{}}Naive forecast\end{tabular}} & \textbf{ForecastBench} & --- & --- & \textbf{0.201} & \textbf{0.008} & \textbf{0.113 (0.009)} & \textbf{0.000} \\
        \begin{tabular}[c]{@{}l@{}}Ensemble models$^\dagger$\end{tabular} & LLM Crowd & \begin{tabular}[c]{@{}l@{}}random set\end{tabular} & \begin{tabular}[c]{@{}l@{}}$\S$\end{tabular} & 0.184 & 0.062 & 0.129 (0.009) & 0.090 \\
        GPT-4o & OpenAI & \begin{tabular}[c]{@{}l@{}}random set\end{tabular} & \begin{tabular}[c]{@{}l@{}}$\ddagger$\end{tabular} & 0.184 & 0.063 & 0.129 (0.009) & 0.090 \\
        \begin{tabular}[c]{@{}l@{}}GPT-4o\end{tabular} & OpenAI & \begin{tabular}[c]{@{}l@{}}Yes\end{tabular} & scratchpad & 0.198 & 0.062 & 0.136 (0.009) & 0.131 \\
        \begin{tabular}[c]{@{}l@{}}Qwen1.5-110B-Chat\end{tabular} & Qwen & \begin{tabular}[c]{@{}l@{}}random set \end{tabular} & \begin{tabular}[c]{@{}l@{}}$\ddagger$\end{tabular} & 0.193 & 0.077 & 0.140 (0.010) & 0.155 \\
        \begin{tabular}[c]{@{}l@{}}Mistral-Large-Latest\end{tabular} & Mistral AI & No & scratchpad & 0.203 & 0.079 & 0.147 (0.007) & 0.192 \\
        \begin{tabular}[c]{@{}l@{}}Claude-2.1\end{tabular} & Anthropic & No & scratchpad & 0.248 & 0.038 & 0.153 (0.011) & 0.224 \\
        \begin{tabular}[c]{@{}l@{}}GPT-4\end{tabular} & OpenAI & No & scratchpad & 0.223 & 0.078 & 0.157 (0.013) & 0.248 \\
        \begin{tabular}[c]{@{}l@{}}GPT-4o\end{tabular} & OpenAI & No & zero-shot & 0.235 & 0.066 & 0.159 (0.011) & 0.258 \\
        \begin{tabular}[c]{@{}l@{}}GPT-4o\end{tabular} & OpenAI & No & scratchpad & 0.235 & 0.070 & 0.160 (0.011) & 0.266 \\
        \begin{tabular}[c]{@{}l@{}}Claude-3-Haiku-20240307\end{tabular} & Anthropic & No & scratchpad & 0.233 & 0.095 & 0.170 (0.007) & 0.325 \\
        Always 0.5 & ForecastBench & --- & --- & 0.250 & 0.107 & 0.185 (0.005) & 0.409 \\ \bottomrule
    \end{tabular}
    }
    {\raggedright\scriptsize\(\dagger\) Median of GPT-4o, Mistral-Large, and Qwen-1.5-110B\\
\(\ddagger\) Superforecaster prompt 3 (see Figure 12)\\\(\S\) All superforecaster prompts (see Figure 10, Figure 11, and Figure 12)\\
See full leaderboard using the anonymized URL link: \url{https://storage.googleapis.com/30e089eb5ad0cff1702d4a5776cc90f3_pub/lm_leaderboard_overall.html}.\\
The z-score reported is relative to the `naive' mean, a representation of one's performance if they forecasted the status quo for all questions; this is because the `naive' mean serves as a control, unaffected by the researchers' decisions around noise and variance.\\
}
\end{table}


==> tables/short_question.tex <==
\begin{table*}[ht!]
  \caption{A sample question with its background, resolution criteria, and key dates. } 
  \vspace{.1cm}
  \label{tab: short-question}
  \centering
  \small
  \renewcommand{\arraystretch}{1.3}
  \setlength\tabcolsep{4pt}
  \begin{tabular}{lp{0.75\textwidth}}
      \toprule
      \textbf{Field} & \textbf{Content} \\
      \midrule
      Question & Will the Cavendish account for less than 50\% of banana exports worldwide before 2035? \\
      Background & Bananas are a well-liked import fruit all over the world, and the Cavendish cultivar has been crushing that market for sixty years. But its rise is literally founded upon the compost heap of the Gros Michel, another cultivar. The so-called “Big Mike” variety had been the leading export towards Europe and North America, but the Panama disease, a fungus belonging to the *Fusarium* clade, killed that. Luckily the Cavendish, grown in the same soil as the wilting Gros Michel, replaced it as *the* banana most of the western world connected with bananas. However, it appears another *Fusarium* rears its spores. Cavendish, with their genetic homogenity (they’re all clones) and sterile nature, aren’t resistant to it, and the fungus is ravaging more and more plantations. There are efforts under way to deal with *Fusarium*, but with various societies’ doubts and misgivings about GMOs, the cure may be viewed as a curse instead. \\
      Resolution Criteria & This question will resolve as Yes if the Cavendish banana accounts for less than 50\% of worldwide annual banana exports in any year from 2018 to 2034 (inclusive). \\
      Key Dates &         Close Date:  2034-12-31 \quad $\mid$ \quad Resolve Date: 2035-01-01 \\
      \bottomrule
  \end{tabular}
\end{table*}

